Combinatorial Group Testing in Presence of Deletions

The study in group testing aims to develop strategies to identify a small set of defective items among a large population using a few pooled tests. The established techniques have been highly beneficial in a broad spectrum of applications ranging from channel communication to identifying COVID-19-infected individuals efficiently. Despite significant research on group testing and its variants since the 1940s, testing strategies robust to deletion noise have yet to be studied. Many practical systems exhibit deletion errors, for instance, in wireless communication and data storage systems. Such deletions of test outcomes lead to asynchrony between the tests, which the current group testing strategies cannot handle. In this work, we initiate the study of non-adaptive group testing strategies resilient to deletion noise. We characterize the necessary and sufficient conditions to successfully identify the defective items even after the adversarial deletion of certain test outputs. We also provide constructions of testing matrices along with an efficient recovery algorithm.

==> relatedw.tex <==
Regnier and Szpankowski: characters of the text are independently generated with fixed probabilities, i.e. a Bernoulli model.  ``Uniform Bernoulli model'' where all the characters occur with the same probability $1/\sigma$. 

Average edit distance between two random strings of length $m$ tends to a constant fraction of $m$ as $m$ grows, but the fraction is not known. 

It holds that for any two strings of length $m$, 
$m - lcs \le ed \le 2(m - lcs)$, 
where $ed$ is their edit distance and $lcs$ is the length of their longest common subsequence. 

Chvatal and Sankoff [1975]: the average LCS is between $m/ \sqrt{\sigma}$ and $m e/\sqrt{\sigma}$ for large $\sigma$, and therefore the average edit distance is between $m (1- e/\sqrt{\sigma})$ and $2m (1 - 1/\sqrt{\sigma})$.

Navarro showed that the average edit distance is larger than $m (1- e/\sqrt{\sigma})$ even for small $\sigma$.
